SafeNet: The Unreasonable Effectiveness of Ensembles in Private Collaborative Learning

Secure multiparty computation (MPC) has been proposed to allow multiple mutually distrustful data owners to jointly train machine learning (ML) models on their combined data. However, by design, MPC protocols faithfully compute the training functionality, which the adversarial ML community has shown to leak private information and can be tampered with in poisoning attacks. In this work, we argue that model ensembles, implemented in our framework called SafeNet, are a highly MPC-amenable way to avoid many adversarial ML attacks. The natural partitioning of data amongst owners in MPC training allows this approach to be highly scalable at training time, provide provable protection from poisoning attacks, and provably defense against a number of privacy attacks. We demonstrate SafeNet's efficiency, accuracy, and resilience to poisoning on several machine learning datasets and models trained in end-to-end and transfer learning scenarios. For instance, SafeNet reduces backdoor attack success significantly, while achieving $39\times$ faster training and $36 \times$ less communication than the four-party MPC framework of Dalskov et al. Our experiments show that ensembling retains these benefits even in many non-iid settings. The simplicity, cheap setup, and robustness properties of ensembling make it a strong first choice for training ML models privately in MPC.

==> RobustBounds.tex <==
\subsection{Ensemble Robustness  Analysis}
%\subsubsection{Bounds on ensemble accuracy}  
\label{sec:bounds}

\smallskip
\myparagraph{Lower bounds on accuracy} We provide lower bounds on SafeNet accuracy, assuming that at most $t$  out  $m$ models in $E$ are poisoned, and the clean models have independent errors, with maximum error rate $p < 1-\threshold$, where $\threshold$ is the filtering threshold.  Crucially, our threat model ensures that there are at least $m-t$ clean models in the ensemble with high probability.  Towards this, we first estimate the minimum number of samples  required in the validation dataset such that all clean models pass the filtering stage of our training phase. Once at least $m-t$ clean models participate in the final ensemble, we provide lower bounds on the SafeNet accuracy as a function of $p$ and $t$. We also provide  bounds for the number of poisoned models $t$ our framework can tolerate as a function of $m$, $\phi$, and $p$.

%\footnote{In the ensemble and collaborative learning settings, independent errors is a natural assumption - if the errors were very well correlated, there would be no benefit to participating in the protocol!}

%Crucially, our threat model ensures that there are at least $m-t$ clean models in the ensemble, where $m$ is the number of models in $E$. We also provide bounds for the number of compromised models $t$ as a function of $m$ and the model error rate~$p$.

\begin{restatable}{lemma}{VS}
	\label{lem:VS} 	 Let  $\Apsc$ be an adversary who poisons $t$ out of $m$ data owners and corrupts $T$ out of $N$ servers,  and thus contributes $t$ poisoned models to  ensemble $E$, given as output by Algorithm 1.
	% Now, given an ensemble $E$ consisting of $m$ models, of which $t$ are poisoned, and a filtering threshold set to $0 \leq \threshold \leq 1$  for a binary classification problem. 
	Assume that  $\pistr$ securely realizes functionality $\FpTrain$ and every clean model in $E$ makes an error on a clean sample  with probability at most  $p < 1- \threshold$,  where $\threshold$ is the filtering threshold. 
	
	If the validation dataset has at least $\frac{(2+\delta)m\log1/\epsilon}{\delta^2(m-t)p}$ samples and $0 \leq t<\frac{m(1-\threshold-p)}{(1-p)}$, then all clean models pass the filtering stage of the training phase with probability at least $1-\epsilon$, where  $\delta = \frac{(1-\threshold)m -t}{(m-t)p}-1$ and $\epsilon$ denotes the failure probability.  
\end{restatable}



%OLD THEOREM
%\begin{restatable}{lemma}{VS}
	
%	Consider an ensemble $E$ consisting of $m$ models, out of which $t$ models are poisoned, and a filtering threshold set to $0 \leq \threshold \leq 1$  for a binary classification problem. 
	%	Consider an ensemble $E$ composed of clean and compromised  models and a filtering threshold $0 \leq \threshold \leq 1$. 
%	We assume that for every clean model in $E$, the probability of making an error  on a clean sample is at most  $p < 1- \threshold$. If the validation dataset has at least $\frac{(2+\delta)m\log1/\epsilon}{\delta^2(m-t)p}$ samples, then all clean models pass the filtering stage of the training phase with probability at least $1-\epsilon$, where  $\delta = \frac{(1-\threshold)m -t}{(m-t)p}-1$, $0 \leq t<\frac{m(1-\threshold-p)}{1-p}$ and $\epsilon$ denotes the failure probability.  
%\end{restatable}


%\begin{lemma}  \label{lem:VS}
%	Consider an ensemble $E$ composed of clean and poisoned/compromised  models and a filtering threshold $0 \leq \threshold \leq 1$. We assume that for every clean model in $E$, the probability of making an error is at most  $p < \threshold$. If the validation dataset has at least $ \frac{(\threshold+p)\log1/\epsilon}{(\threshold-p)^2}$ samples, then all clean models pass the filtering stage of the training phase with probability at least $1-\epsilon$, where $\epsilon$ denotes the failure probability.  
%\end{lemma}

\begin{proof}
	The proof is deferred to Appendix~\ref{proof:VS}.
\end{proof}


\begin{restatable}{theorem}{LB} \label{thm:LB}
Assume that the conditions in Lemma~\ref{lem:VS} hold against  adversary $\Apsc$ poisoning at most $ t < \frac{m}{2}\frac{1-2p}{1-p}$ owners and that the errors made by the clean models are independent.
	% Let $m$ be the total models in the filtered ensemble $E_f$, of which $t$ models are compromised.
	Then $E$  correctly classifies new samples with probability at least $ p_c = (1- \epsilon) \left(1 - e^{-\frac{\delta'^2\mu'}{2+\delta'}}\right)$, where $\mu' = (m-t)p$ and $\delta' = \frac{m-2t}{2\mu'} - 1$.
\end{restatable}


\begin{proof}
	The proof is deferred to Appendix~\ref{proof:LB}.
\end{proof}

The theorem provides theoretical lower bounds on the test accuracy of our  SafeNet framework as a function of the maximum error probability among the clean models. Later in Section \ref{subsec:Params}, we provide details on how to set these parameters in practice and compare these theoretical bounds with  our experimental results.
% and analyze the tightness of these bounds.

%The guarantee provided by Theorem~\ref{thm:LB} can be difficult to visualize. To address this, 


%The right plot in Figure~\ref{fig:LB_plots} shows the lower bound on SafeNet accuracy, given there were minimum required samples in the validation set such that all clean models cleared the filtering stage in the training phase. We observe, as the model errors decrease ($p=0.01$), \safenet can tolerate more corruption while achieving a high accuracy. Note that these are lower bounds, as we assumed that the $t$ poisoned models misclassify all the samples.  Our results in Section~\ref{sec:exp} show higher robustness for \safenet against backdoor and targeted  attacks.  


%\safenet achieves high accuracy up to 5 (out of 20) owners with poisoned data, even for large model error rates. As the model errors decrease ($p=0.01$), \safenet can tolerate more corruption. Note that these are lower bounds, as we assumed that the $t$ corrupted models are mis-classifying all the samples.  Our results in Section~\ref{sec:exp} show higher robustness for \safenet for backdoor and targeted poisoning attacks.  

\begin{comment}

\begin{figure}[h]
		\caption{ \small Minimum number of samples in the validation dataset as a function of maximum error probability $p$ and number of poisoned owners  $t$ across $m = 20$ data owners in the ensemble (left). We set the filtering threshold $\threshold$ and  failure probability $\epsilon$  to $0.5$ and $0.01$ respectively. Lower bound on \safenet accuracy for varying number of poisoned models $t$ and maximum error probability $p$ (right).}
	%given the number of samples in the validation set are at least as  shown in the left plot.} 	
\label{fig:LB_plots}
	\centerline{
		\includegraphics[width=0.25\textwidth]{CV_size}%
		\includegraphics[width=0.25\textwidth]{EAcc}%
	}
	\end{figure}
\end{comment}

%---------------------------------------

\begin{comment}

\begin{figure}[h!] 
%	\vspace{-3mm}
\centering
\caption{\small Lower bound plots of \safenet accuracy for varying number of compromised models $t$ and maximum error probability $p$ across $m = 20$ models in the ensemble.}
\label{fig:LB_plots}

\includegraphics[scale=0.5]{LB_Plot.pdf}
%	\vspace{-4mm}
\end{figure}
\end{comment}

\smallskip
\myparagraph{Certified Prediction}
Theorem~\ref{thm:LB} demonstrates that SafeNet's accuracy on in-distribution data will not be compromised by poisoning. However, we now show that we can also certify robustness to poisoning on a per-sample basis for arbitrary points, inspired by certified robustness techniques for adversarial example robustness~\cite{cohen2019certified}. In particular, Algorithm 2 describes a method for certified prediction against poisoning, returning the most common class $y$ predicted by the ensemble on a test point $x$, as well as a bound on the number of poisoning owners $t$ which would be required to modify the predicted class.
\begin{comment}
\begin{algorithm}
	\begin{algorithmic}
		\smallskip
		\State Input: $m$ data owners; Ensemble of models $E = \lbrace \fm_i \rbrace_{i=1}^{m}$; Testing point $x$; Differential Privacy parameter $\epsilon$.
		\State $\textsc{Counts} = \sum_{i=1}^m \fm_i(x) + \textsc{DPNoise}(\epsilon)$  \Comment{$\fm_i(x)$ one-hot}
		\State $y, c_y = \textsc{MostCommon}(\textsc{Counts})$ \Comment{most common predicted class with noisy count}
		\State $y', c_{y'} = \textsc{SecondMostCommon}(\textsc{Counts})$ \Comment{second most common predicted class with count}
		\State $t = \lceil(c_y-c_{y'})/2\rceil - 1$
		\State \Return $y, t$
	\end{algorithmic}
	\caption*{{\bf Algorithm 2} Certified Private Prediction $\textsc{CertPred}~(E,x)$} 
\end{algorithm}


\begin{restatable}{theorem}{RP} \label{thm:robustpredcorrect} Let $E$ be an ensemble of models trained on  datasets $D=\{D_1,\dots,D_m\}$. Assume that on an input $x$, the ensemble generates prediction $y=E(x)$ and Algorithm 2 outputs $(y, t)$. Moreover, assuming an adversary $\Apsc$ who poisons at most $t$ data  owners, the resulting $E'$ trained on poisoned data $D'$ generates the same prediction on $x$ as $E$: $E'(x)=y$.

%(where $|D' \setminus D| \le t-1$) 

%	If the Robust Prediction method from Algorithm~\ref{alg:robustpred}  outputs $y, t$ on input $x$, then no set of $t-1$ corrupt owners could have changed the prediction of $x$ to $y'$.
\end{restatable}

\begin{proof}
	%We keep the notation from Algorithm~\ref{alg:robustpred}. 
	If an adversary's goal were to cause $y'$ to be predicted on input $x$, their most efficient strategy is to flip $y$ predictions to $y'$. If $y$ were the ensemble prediction, it must have at least $\lfloor\frac{c_y+c_{y'}}{2}\rfloor$ model predictions, and the second most common prediction $y'$ would have at most $\lfloor\frac{c_y+c_{y'}}{2}\rfloor$ model predictions. Corrupting these predictions then requires flipping at least $(c_y-c_{y'})/2$ predictions from $y$ to $y'$. Overall, this requires at least $\lceil(c_y-c_{y'})/2\rceil$ poisoned data owners. Thus, an adversary poisoning  at most $t = \lceil(c_y-c_{y'})/2\rceil-1$ data owners still generates the same prediction $y$ on $x$.
\end{proof}
\end{comment}

==> SafenetDetails.tex <==
\subsection{\safenet Overview}\label{sec:SNoverview}
%\begin{comment}
\begin{figure*}[t] 
	%	\vspace{-3mm}
	%\centering
	\includegraphics[scale=0.3]{SafeNet_Overview.pdf}
	\caption{Overview of the Training and Testing phases of the \safenet Framework.}
	\label{fig:EF}
	%	\vspace{-4mm}
\end{figure*}
%\end{comment}


Given our threat model in Figure~\ref{fig:AS}, existing PPML  frameworks provide security against an $\Asoc$ adversary, but they are not designed to handle an  adversary of type  $\Apsc$. We show experimentally in Section~\ref{sec:exp} that PPML frameworks for private training are susceptible to data poisoning attacks.  While it would be possible to remedy this by implementing specific poisoning defenses (see Section~\ref{sec: otherDefenses} for a discussion of these approaches), we instead show that it is possible to take advantage of the bounded poisoning capability of $\Apsc$ to design a more general and efficient defense. Intuitively, existing approaches train a single model on all local datasets combined, causing the model's training set to have a large fraction of poisoned data ($t/m$), which is difficult to defend against. Instead, we design SafeNet, a new framework which uses ensemble models to realize our threat model and provide security against $\Apsc$. In addition to successfully mitigating data poisoning attacks, SafeNet provides more efficient training than existing PPML and comparable prediction accuracy.


 %Existing privacy-preserving ML training frameworks are unequipped with the necessary tools to mitigate data poisoning attacks introduced by the poisoned data owners. In order to address this issue, we propose an alternate training method which not only gives prediction accuracy comparable to the traditional model and efficient training, but is also able to successfully mitigate data poisoning attacks.  

Figure~\ref{fig:EF} provides an overview of the training and testing phases of SafeNet. \safenet trains an ensemble $E$ of multiple models in protocol $\pistr$, where each model $\fm_k \in E$ is trained locally by the data owner $\usr_k$ on their dataset. This partitioning prevents poisoned data from contributing to more than $t$ local models. Each data owner samples a local validation dataset and trains the local model $\fm_k$ on the remaining data. The local models and validation datasets are secret shared to the outsourced servers. We note that this permits arbitrarily corrupted models, and poisoned validation datasets, but SafeNet's structure still allows it to tolerate these corruptions. In the protocol running inside the MPC, the servers jointly implement a filtering stage for identifying models with low accuracy on the combined validation data  (below a threshold $\phi$) and excluding them from the ensemble. The output of training is a secret share of each model in the trained ensemble $E$. Note that exclusion in this case does not mean explicitly removing the model from the ensemble, but, instead, not including the model's prediction in the testing voting procedure. Later in Section  \ref{sec:sectrain}, we show a way to realize the filtering stage without revealing which models is excluded from the final ensemble.

%Towards this goal, the servers compute the validation accuracy on the global validation set $\CV$ and remove models with accuracy lower than a fixed threshold $\phi$. 

In the prediction phase, SafeNet implements protocol $\piPred$, which generates the prediction $y_k$ of each shared model $\fm_k$ on test input $x$ inside the MPC. The servers  jointly perform majority voting to determine the most common predicted class $y$ on input $x$, using only the models which pass the filtering stage.

%In addition, each data owner contributes a small fraction of its dataset to construct a common validation dataset, which we use to compute accuracy for each ensemble model. We use this phase in order to filter models from the ensemble that have low accuracy on the common validation dataset. 
%We will show that this filtering procedure prevents poisoning availability attacks.
% The remaining models in the ensemble are secret shared among the servers participating in the SOC protocol. 
%The filtered ensemble is then used to generate a prediction where the servers run an MPC protocol to perform majority voting over the individual models predictions.  

Our \safenet protocol leverages our threat model, which assumes that only a set of at most $t$ out of $m$ data owners are poisoned. This ensures that an adversary only influences a limited set of models in the ensemble, while existing training protocols would train a single poisoned global model. We provide bounds for the exact number of poisoned owners $t$ supported by our ensemble in Theorem~\ref{thm:LB}. Interestingly, the bound depends on the number of data owners $m$, and the maximum error made by a clean model in the ensemble.  The same theorem also lower bounds the probability that the ensemble predicts correctly under data poisoning performed by the $t$ poisoned owners, and we validate experimentally that, indeed, \safenet provides resilience to stealthy data poisoning attacks, such as backdoor and targeted attacks. Another advantage of \safenet is that the training time to execute the MPC protocols in the SOC setting is drastically reduced as each $\fm_k \in E$ can be trained locally by the respective owner. 
%
We detail below the algorithms for training and prediction in SafeNet. 

%The only protocols implemented in the MPC are: (1) Ensemble Filtering; and (2) \safenet prediction, which we detail below.

%Concretely, our approach is to build an ensemble $E$ where each model $\fm_k \in E$ is trained on the dataset $ \ld_k \in \fd$ possessed by the data owner $\usr_k$. This constructed $E$ replaces $\fm$, which was earlier trained over the combined dataset $\fd$. The advantages of our approach are two fold:


%For simplicity, we describe the working of our SafeNet framework as a two step process:
%\begin{itemize}
%	\item [--] The first step computes the {\OB} accuracy of each model which  help us to differentiate between the behavior of an honest from a corrupt owner.

%	\item[--] The second step compares each model's {\OB} accuracy with a pre-agreed threshold to remove poisoned or poorly performing models from $E$.
%\end{itemize}



\begin{comment}
\begin{figure}[h!]
\caption{Schematic representation of SafeNet Framework}
\label{fig:EF}

\vspace{2mm}
\begin{tikzpicture}[node distance= 1cm]

\node(maldo)[draw, text centered, text width=2.7cm,fill=orange!70, font = \small, xshift = -4cm] {Corrupt owners \\ Dataset and Models};

\node(hdo)[draw, text centered, text width=2.7cm,right of  = maldo, font = \small, xshift = 4.2cm,fill=cyan!55] {Honest owners \\ Dataset and Models};

\node(uoob)[draw, text centered, rounded corners, text width=2.7cm,below of  = maldo, font = \small, xshift = 2.6cm,yshift = -0.4cm, fill=white!60] {$\OB$ Accuracy};

\node(tc)[draw, text centered,rounded corners, text width=2.7cm,font = \small, below of  = uoob, fill=white!60] {Threshold Comparison};

\node(fe)[draw, text centered, rounded corners, text width=2.7cm,below of  = tc, font = \small, fill=white!60] {Final Ensemble};

\node(soc)[soc,  minimum height=2.8cm, above of = uoob, label= {\footnotesize Ensemble Filtering}, yshift = -2cm]{};

\path[draw,-latex,  bend right] (maldo) edge (uoob);
\path[draw,-latex,  bend left] (hdo) edge (uoob);
\path[draw,-latex] (uoob) edge (tc);
\path[draw,-latex] (tc) edge (fe);
\end{tikzpicture}

\end{figure}
\end{comment}


\subsection{\safenet Training} \label{sec:train}

To train the ensemble in SafeNet, we show our proposed ensemble method in Algorithm 1. We  discuss the realization in MPC  later in Section~\ref{sec:mpc_inst}. Each owner $\usr_k$ separates out a subset of its training dataset $\cv{k} \in \ld_k$ and then trains its model $\fm_k$ on the remaining dataset $\ld_k \setminus \cv{k}$. The trained model $\fm_k$ and validation dataset $\cv{k}$ is then secret-shared to the servers. The combined validation dataset is denoted as $\CV = \bigcup\limits_{i=1}^{m} \cv{i}$. We assume that all users contribute equal-size validation sets to $\CV$. During the filtering stage inside the MPC, the validation accuracy $\valacc$ of each model is jointly computed on $\CV$. If the resulting accuracy for a model is below threshold $\threshold$, the model is excluded from the  ensemble. 

%\newcommand{\pistr}{\ensuremath{\Pi_\mathsf{str}}}

The  filtering step is used to separate the models with low accuracy, either contributed by a poisoned owner, or by an owner holding non-representative data for the prediction task.
%prevents against an adversary contributing a low-accuracy model (e.g., a model trained on random labels of the data), or against an owner holding a non-representative dataset for the learning task. 
  Under the assumption that the majority of owners are honest, it follows that the majority of validation samples are correct. If  $\usr_k$ is honest, then the corresponding $\fm_k$ should have a high validation accuracy on $\CV$, as the corresponding predicted outputs would most likely agree with the samples in $\CV$. In contrast, the predictions by a poisoned model $\fm_k$ will likely not match the samples in $\CV$.  In Section~\ref{sec:bounds}, we compute a lower bound on the size of the validation dataset as a function of  the number of poisoned owners $t$ and filtering threshold $\threshold$, such that all clean models pass the filtering stage with high probability even when a subset of the cross-validation dataset $\CV$ is poisoned. 

Given protocol $\pistr$ that securely realizes Algorithm 1 inside the MPC (which we will define later in Section~\ref{sec:mpc_inst}), we argue security as follows:

\begin{restatable}{theorem}{SPtrain} \label{thm:SNtrain}
Protocol $\pistr$ is secure against  adversary $\Apsc$ who poisons $t$ out of $m$ data owners and  corrupts $T$ out of $N$ servers.
\end{restatable}

\noindent
The proof of the theorem will be given in Appendix~\ref{app:secproof} after we introduce all the details of MPC instantiation and how  protocol $\pistr$ securely realizes $\FpTrain$ in Section \ref{sec:sectrain}. 

%Note that, the inputs to $\FpTrain$ with respect to each owner $\usr_i$ would be dataset $D_i = \cv{i}$ and auxiliary input $a_i = \fm_i$.

%This way, we can set the threshold value $\threshold$ according to the number of poisoned owners $t$ and the expected worst-case error by the clean models. We discuss the impact of choice of $\threshold$ on ensemble filtering stage and later in \cref{sec:fashion_nn}.

%\commentH{Add theorem here stating safenet training securely realizes $\FpTrain$}.


%The "$\OB$ (Owner-Out-Of-Bag)" accuracy for a given owner $\usr_k$ is calculated by computing the predictions of her/his trained model $\fm_k$ over a dataset $\fd_{ob}$, followed by comparing the predicted outputs to their respective true labels. 

%Thus, for each owner $\usr_k$, dataset $\fd_{ob}$ acts a cross-validation/$\OB$ dataset and  will have a $\OB$ accuracy associated with her/his model $\fm_k$. 
%The reason behind using $\OB$ accuracy as a parameter for selection is  based on the prior knowledge that the  $\fd_{ob}$ comprises of data samples from honest owners in majority. If  $\usr_k$ is honest then the corresponding $\fm_k$, when tested against $\fd_{ob}$ should have a high $\OB$ accuracy as the corresponding predicted outputs would probably agree with most of the true labels associated with the samples in $\fd_{ob}$, as majority of the samples in $\fd_{ob}$ constitute the honest owners $\OB$ dataset. A similar argument can be made for a corrupt $\usr_k$ where her/his predicted outputs will mismatch with the labels associated to the samples in $\fd_{ob}$. 

%This strategy works against certain types of attacks (for eg. availability attacks)  where the goal of the adversary is to decrease the accuracy of the ensemble $E$ . Our filtering strategy will remove such models as each corrupt owner can reduce the accuracy of $E$, only by causing it's own model to perform poorly which will highly likely have its $\OB$ accuracy less than a sepcified threshold $T$.
%
% Similarly, if $\usr_k$ is corrupt, $\pred_{\sss{\ld_i}}$ will most likely agree with the labels associated with the samples of other corrupt users but may have many mismatches with the labels associated to the samples submitted by the honest users (who are in majority). Thus on an average the u-OOB accuracy for a $\lm_i$ submitted by an honest user is likely to be more than the u-OOB accuracy for a $\lm_i$ of a corrupt user. We concretize our claims later in section \ref{sec:RPA}, where we observe the variation in u-OOB accuracy for an honest and corrupt user with change in pollution amount. 

%\begin{comment}


\begin{algorithm}[t]
	
	\caption*{{\bf Algorithm 1} SafeNet Training Algorithm} \label{alg:ensemblefiltering}
	\begin{algorithmic}
		
		%\smallskip
			\State Input: $m$ data owners, each owner $\usr_k$'s   dataset $\ld_k$. 	
		%		, owner-out-of-bag data  $\fd_{ob} = \bigcup\limits_{i=1}^{m} \ld^{ob}_i$ and threshold $T$.				
		%		ensemble of models $ E = \lbrace \fm_i \rbrace_{i=1}^{m}$
		%\smallskip
			 \Comment{\footnotesize Owner's local computation in plaintext format} 
			\State -- For $k \in [1,m]:$	
			\begin{itemize}
				\item[-] Separate out $\cv{k}$ from $\ld_k$. Train $\fm_k$ on $\ld_k \setminus \cv{k}$.
				\item[-] Secret-share $\cv{k}$ and $\fm_k$ to servers.
			\end{itemize}
		
		%\smallskip
%		\State Owners also secret-share a pre-agreed threshold $\threshold$ to the servers.
		
		%\smallskip
			\Comment{\footnotesize MPC computation in secret-shared format}
			\State -- Construct a common validation dataset $\CV = \cup_{i=1}^{m} \cv{i}$ and collect ensemble of models $ E = \lbrace \fm_i \rbrace_{i=1}^{m}$
		
			\State -- Initialize a vector $\valvec$ of zeros and of size $m$. 
		
		%\smallskip
			\State  -- For $k \in [1,m]:$ \Comment{\footnotesize Ensemble Filtering}
			\begin{itemize}
				\item[-] $\valacc_k = Accuracy(\fm_k, \CV)$ \Comment{\footnotesize Compute validation accuracy of $\fm_k$ over $\CV$. }
			
%			\item[-] $\textsc{Preds}_k = \fm_k(\fd_{ob})$  \Comment{Compute output predictions of $\fm_k$ over $\fd_{ob}$. }
			
			%\item[-] $\text{O}^3\text{B}_\text{k} = \frac{1}{\abs{\fd_{ob}}} \sum_{i=1}^{\abs{\fd_{ob}}}\mathbbm{1}[\textsc{Preds}^i_k == \text{y}^i_{\fd_{ob}}]$ \Comment{Compute $\OB$ accuracy of the model.}
			
				\item[-] If $\valacc_k> \threshold$: \Comment{\footnotesize Compare against threshold} 
				\begin{itemize}
					\item[--] Set $\valvec_k = 1$   \Comment{\footnotesize Set $k^{th}$ position in $\valvec$ to 1} 
				
				%	\item[-] $ \textsc{Ensemble} = \textsc{Ensemble} \cup  \fm_i$   \Comment{add models in final ensemble if u-OOB accuracy greater than threshold}
				\end{itemize}			
			
			\end{itemize}
		%\smallskip
			\State \Return $E$ and $\valvec$
		\end{algorithmic}
%		\caption{SafeNet Training Algorithm}{}
\label{alg:train}
\end{algorithm} 


\begin{comment} 
\begin{algorithm}
\begin{algorithmic}

\State Input: number of data owners $m$, ensemble of models $ E = \lbrace \fm_i \rbrace_{i=1}^{m}$ , owner-out-of-bag data  $\fd_{ob} = \bigcup\limits_{i=1}^{m} \ld^{ob}_i$ and threshold $T$.
%\State $\textsc{Ensemble} = \{\}$

\State For $k \in [1,m]:$
\begin{itemize}
\item[-] $\textsc{Preds}_k = \fm_k(\fd_{ob})$  \Comment{Compute output predictions of $\fm_k$ over $\fd_{ob}$. }

\item[-] $\text{O}^3\text{B}_\text{k} = \frac{1}{\abs{\fd_{ob}}} \sum_{i=1}^{\abs{\fd_{ob}}} \textsc{Preds}^i_k == \text{y}^i_{\fd_{ob}}$ \Comment{Compute $\OB$ accuracy of the model.}

\item[-] If $\OB_k< T$: 
\begin{itemize}
\item[--] Remove $\fm_i$ from ensemble $E$.

%	\item[-] $ \textsc{Ensemble} = \textsc{Ensemble} \cup  \fm_i$   \Comment{add models in final ensemble if u-OOB accuracy greater than threshold}
\end{itemize}			

\end{itemize}


\State \Return $E$
\end{algorithmic}
\caption{SafeNet Training Algorithm \alina{I think this algorithm should start from input the datasets, Then we need to add training  models locally and construction of validation data.}}
\label{alg:ensemblefiltering}
\end{algorithm} 

\begin{algorithm}
\begin{algorithmic}

\State Input: number of model providers (data owners) $p$, number of models per provider $q$, set of models $ E = \lbrace \fm_i \rbrace_{i=0}^{qp-1}$ , combined data from model providers $\fd = \bigcup\limits_{k=1}^{p} \ld_k$ and threshold $T$.
%\State $\textsc{Ensemble} = \{\}$

\State For $k \in [p]:$
\begin{itemize}
\item[] For $i \in [(k-1)q, kq-1]:$
\begin{itemize}
\item[-] $\textsc{Preds}_i = \fm_i(\dataset_{\sss{\fd}} / \dataset_k)$

\item[-] If $\text{O}^3\text{B}~\textsc{(Preds}_i,~ \lbl_{\sss{\fd}} / \lbl_k) < T$: 
\begin{itemize}
\item[--] Remove $\fm_i$ from set $E$.

%	\item[-] $ \textsc{Ensemble} = \textsc{Ensemble} \cup  \fm_i$   \Comment{add models in final ensemble if u-OOB accuracy greater than threshold}
\end{itemize}			

\end{itemize}
\end{itemize}


\State \Return $E$
\end{algorithmic}
\caption{Ensemble Filtering Algorithm}
\label{alg:ensemblefiltering}
\end{algorithm}
\end{comment}


==> SecDef.tex <==
In this section, we first describe the adversarial model considered in state-of-the-art privacy preserving ML training frameworks. We then extend this adversarial model by allowing the adversary to poison the training data of a subset of owners.  Finally, we provide an overview of the \safenet framework, discuss its realization as a collection of MPC protocols, and detail the underlying MPC building blocks required to implement \safenet in a privacy-preserving manner.

%We use $\fd$ to denote the combined dataset of all the participating users, where $\fd = (\dataset_{\sss{\fd}}, \lbl_{\sss{\fd}})$. Matrix $\dataset_{\sss{\fd}}$ represents a feature matrix where the number of rows represent the total number of training samples submitted by all the users combined and $\lbl_{\sss{\fd}}$ denotes the corresponding vector of true labels. We use $\ld_i = {(\dataset_i, \lbl_i)}$ to denote a subset of the combined dataset ($\ld_i \subset \fd$).

%In the real world it is quite feasible for $\Adv$ to poison the training data of the owners it has control over and such attacks would go undetected while training under the standard MPC frameworks. As a consequence, we restructure the threat model to accommodate our new adversary to poison the training data of the corrupt owners. 


% Additionally, some training frameworks \cite{..} also allow the final trained model to be reconstructed towards the data owners. Again, this is not a good practice as recent works\cite{..} have shown that it is possible to extract training data from a model. This would directly violate the security definition described in Section.\ref{sec:SecDef}, of the adversary not having knowledge of the honest owners dataset. Ergo, it is recommended for the final model $\fm$ to either remain secret-shared among the outsourced servers or to be sent back to owners in an encrypted/secret-shared format.     



\subsection{Threat Model} \label{sec:threat_model}

{
	\begin{figure}[t ]
		\vspace{-1.5mm}	
		\begin{tikzpicture}[node distance= 0.7cm]
			\node(maldo1)[maldo]{ \footnotesize $\usr_1$ };
			%\node(maldo2)[maldo, below of=maldo1]{Data owner 2};
			\node(maldoi-1)[maldo, below of=maldo1]{\footnotesize $\usr_t$ };
			\node(hdoi)[hdo, below of=maldoi-1]{\footnotesize $\usr_{t+1}$ };
			\node(hdom)[hdo, below of=hdoi]{\footnotesize $\usr_m$ };
			
			\node(mals1)[malserver, right of = maldo1, xshift=4.6cm, yshift = -0.3cm]{\footnotesize S$_1$};
			
			\node(mals2)[malserver, right of = mals1, yshift = -0.8cm]{\footnotesize S$_2$};
			
			\node(malsT)[malserver, below  of = mals1, yshift = -1.0cm]{ \footnotesize S$_{\scaleto{T}{3pt}}$};
			
			\node(hsT1)[hserver, left  of = malsT, xshift = -0.4cm]{S$_{\footnotesize \scaleto{T+1}{3pt}}$};
			
			\node(hsN)[hserver, xshift = -0.4cm , left of = mals1]{S$_{\footnotesize \scaleto{N}{3pt}}$};
			
			\node(hsN1)[hserver, yshift = -0.8cm , left of = hsN]{S$_{\footnotesize \scaleto{N-1}{3pt}}$};
			
			\node(soc)[soc, left of = hsN, label= {\footnotesize SOC Paradigm}, xshift = 1.25cm, yshift = -0.85cm]{};
			
			\node(nota)[nota, below of = soc, xshift = - 2.1cm, yshift = -1.1cm]{};
			
			\node(mdnota)[mdnota, label = right: {\footnotesize Poisoned}, left of = nota, xshift = -2.3cm]{};
			\node(msnota)[msnota, right of = mdnota, label = right: {\footnotesize Corrupted}, xshift = 1.78cm]{};
			\node(hnota)[hnota, right of = msnota,label = right: {\footnotesize Honest}, xshift = 1.8cm]{};
			
			\path (maldo1) -- node[auto=false]{\ldots} (maldoi-1);
			%\path (maldoi-1) -- node[auto=false]{\ldots} (hdoi);
			\path (hdoi) -- node[auto=false]{\ldots} (hdom);
			\path (hdoi) -- node[auto=false]{\ldots} (hdom);
			
			\path[draw, densely dotted,  bend left] (mals2) edge (malsT);
			\path[draw, densely dotted,  bend left] (hsT1) edge (hsN1);
			
			\draw[sarrow](mals1) -- (mals2);
			\draw[sarrow](mals1) -- (malsT);
			\draw[sarrow](mals1) -- (hsT1);
			\draw[sarrow](mals1) -- (hsN1);
			\draw[sarrow](mals1) -- (hsN);
			
			\draw[sarrow](mals2) -- (malsT);
			\draw[sarrow](mals2) -- (hsT1);
			\draw[sarrow](mals2) -- (hsN1);
			\draw[sarrow](mals2) -- (hsN);
			
			\draw[sarrow](malsT) -- (hsT1);
			\draw[sarrow](malsT) -- (hsN1);
			\draw[sarrow](malsT) -- (hsN);
			
			\draw[sarrow](hsT1) -- (hsN1);
			\draw[sarrow](hsT1) -- (hsN);
			
			\draw[sarrow](hsN1) -- (hsN);
			
			\draw[darrow](maldo1) -- (soc);
			\draw[darrow](maldoi-1) -- (soc);
			\draw[darrow](hdoi) -- (soc);
			\draw[darrow](hdom) -- (soc);
		\end{tikzpicture}
		\caption{Threat model considered in our setting. The adversary $\Apsc$ can poison at most $t$ out of $m$ data owners and corrupt at most $T$ out of $N$ servers participating in the MPC computation. $\usr_i$ and $\srvr_j$ denote the $i^{th}$ data owner and $j^{th}$ server respectively.}
		\label{fig:AS}
		\vspace{-1.5mm}
\end{figure}}


%\myparagraph{Notations}
%We introduce notations for a better understanding of the following sections.  A single training/testing sample is expressed as $(\ssample_i, \slbl_i)$, where $\ssample_i$ is the input feature vector and $\slbl_i$ is its corresponding true label. We use $\ld_k = (\dataset_{\sss{k}}, \lbl_{\sss{k}})$ to denote dataset of data owner $\usr_k$ participating in the training process. Matrix $\dataset_{\sss{k}}$ represents a feature matrix where the number of rows represent the total training samples possessed by $\usr_k$ and $\lbl_{\sss{k}}$ denotes the corresponding vector of true labels. When assigning a variable/value $y$ to variable $x$, we use the notation $x = y$, while $x == y$ denotes the statement that the two are of equal value. Also, $[m,n]$ denotes a short hand notation to represent a continuous range of values $\{m,\ldots,n\}$. 
% Notation $\fd = (\dataset_{\sss{\fd}}, \lbl_{\sss{\fd}})$ denotes the combined dataset of all participating users.

\myparagraph{Setup} We consider a set of $m$ data owners $C= \cup_{k=1}^{m} \usr_k$ who wish to train a joint machine learning model $\fm$ on their combined dataset $\fd =  \cup_{k=1}^{m} \ld_k$. We adopt the Secure Outsourced Computation (SOC) paradigm~\cite{MohasselZ17, MR18, WaghGC18, PS20, BCPS20, RRKCGRS20, WTBKMR21, AEV21, DEK20, DEK21} for training model $\fm$ privately, where the owners secret-share their respective datasets to a set of  outsourced servers, who enact the role of mutually distrusting  parties in the MPC and execute the necessary protocols to train $\fm$. The final output after execution of these protocols is a trained model in secret-shared format among the servers.  
A single training/testing sample is expressed as $(\ssample_i, \slbl_i)$, where $\ssample_i$ is the input feature vector and $\slbl_i$ is its corresponding true label or class. We use $\ld_k = (\dataset_{\sss{k}}, \lbl_{\sss{k}})$ to denote dataset of data owner $\usr_k$ participating in the training process. Matrix $\dataset_{\sss{k}}$ denotes a feature matrix where the number of rows represent the total training samples possessed by $\usr_k$ and $\lbl_{\sss{k}}$ denotes the corresponding vector of true labels.

\smallskip
%\noindent
\myparagraph{Adversary in the SOC} Given  a set $S = \{\srvr_1,\ldots,\srvr_N\}$ of outsourced servers, we define an adversary $\Asoc$,  similar to prior work~\cite{MohasselZ17, MR18, RRKCGRS20, WTBKMR21, AEV21, DEK21}.  $\Asoc$ can statically corrupt a  subset $S_T \subset S$ of servers of size at most $T<N$. The exact values of $N$ and $T$ are dependent on the  MPC protocols  used for training the ML model privately. For instance, we experiment with two-party, three-party, and four-party protocols with one corrupt server. MPC defines two main adversaries: i) \emph{Semi-honest}: Adversary follows the described protocol, but tries to derive additional information from the messages received from other parties during the protocol; ii) \emph{Malicious}: Adversary has the ability to arbitrarily deviate during the execution of the protocol. For our security proofs, we assume the adversary to be semi-honest, but our approach can be extended to malicious adversaries.

\smallskip
%\noindent
\myparagraph{Security Definition} MPC security is defined using the real world - ideal world paradigm~\cite{C00}.
%Security is defined by comparing a real and ideal interaction. 
In the real world, parties participating in the MPC interact during the execution of a protocol $\pi$ in presence of an adversary $\Adv$. Let $\mathsf{REAL}[\mathbb{Z}, \Adv, \pi, \lambda]$ denote the output of the environment $\mathbb{Z}$ when interacting with $\Adv$ and the honest parties, who execute $\pi$ on security parameter $\lambda$. This interaction is called the real-world interaction. Effectively, $\mathsf{REAL}$ is a function of the inputs/outputs and messages sent/received during the protocol. In the ideal world, the parties simply forward their inputs to a trusted functionality $\mathcal{F}$ and forward the functionality's response to the environment.
Let $\mathsf{IDEAL}[\mathbb{Z}, \Sim, \mathcal{F}, \lambda]$ denote the output of the environment $\mathbb{Z}$ when interacting with adversary $\Sim$ and honest parties who run the  protocol in presence of $\mathcal{F}$ with security parameter $\lambda$. The security definition states that the views of the adversary in the real and ideal world are indistinguishable: 
% We now define security for our threat model as follows:

\begin{definition} \label{def:mpc_sec}
	A  protocol $\pi$ securely realizes  functionality $\mathcal{F}$   if for all environments $\mathbb{Z}$ and any adversary of type $\Asoc$, which  corrupts a subset $S_T$ of servers of size at most $T < N$ in the real world, then there exists a simulator $\Sim$ attacking the ideal world, such that $\mathsf{IDEAL}[\mathbb{Z}, \Sim, \mathcal{F}, \lambda] \approx \mathsf{REAL}[\mathbb{Z}, \Asoc, \pi, \lambda]$.
\end{definition}

%-----------------Old Definition-------------------------------
%\begin{definition}
%	A training protocol $\pitrain$ securely realizes our functionality $\FpTrain$  if for all environments $\mathbb{Z}$ and any adversary of type $\Apsc$, which poisons a subset $D_t$ of datasets of size at most $t<m$ and corrupts a subset $S_T$ of servers of size at most $T < N$ in the real world, then there exists a simulator $\Sim$ attacking the ideal world, such that $\mathsf{IDEAL}[\mathbb{Z}, \Sim, \FpTrain, \lambda] \approx \mathsf{REAL}[\mathbb{Z}, \Apsc, \pitrain, \lambda]$ 
%\end{definition}



%Many training frameworks~\cite{...} have been designed to tackle privacy-preserving training of ML algorithms, of which  several  have been constructed for the SOC paradigm~\cite{..}.



%Given a set of $m$ data owners and a set of $N$ severs, the threat model  in prior works ~\cite{MohasselZ17, MR18, WaghGC18, PS20, BCPS20, RRKCGRS20, WTBKMR21, AEV21, DEK20, DEK21} considers an adversary $\Asoc$  who can corrupt an arbitrary subset of data owners and  a fixed $T < N$  subset of servers depending on the specification of  on the  MPC protocols that are used for training the model $\fm$.

%The security definition requires that the adversary only learns the data of the corrupted owners and no information about the remaining honest owners' data and the final trained model is revealed.  Figure \ref{fig:ideal_ml} provides description of the ideal functionality $\FTrain$ that the aforementioned frameworks realize to train a model privately.

%\Apsc

%We provide a brief description of the security definition here, but refer the reader to \cite{Canetti00, Can01} for more technical details.

%\begin{comment}
\begin{comment}
\begin{systembox}{$\FTrain$}{Ideal Functionality for ML training}{func:ml}   \label{fig:ideal_ml}
	\algoHead{Parameters:} A set $U = \{\usr_1,\ldots,\usr_m\}$ of data owners with training datasets $\ld_1, \ldots, \ld_m$ respectively and a set $S = \{S_1,\ldots,S_N\}$ of outsourced servers.
	
	\smallskip
	\algoHead{Uploading Data:}  On input $\ld_i$ from $\usr_i$, store $\ld_i$ internally.
	
	\smallskip
	\algoHead{Computation}: On input ML training algorithm $f$ from one of the servers, compute $(z_1,\ldots, z_N)$ = $f(\ld_1, . . . , \ld_m)$ and send  $z_i$ to server $S_i$, where $z_i$ denotes a secret-share of the trained model in appropriate format.
	
	\smallskip
	%	This step can be repeated multiple times with different algorithms.
\end{systembox}
\end{comment}

%However, the  threat model does not take into consideration the quality of the underlying training data and assumes that the datasets contributed   towards training by the corrupted data owners is not poisoned. This is a strong assumption given the effect of  data poisoning attacks  on trained models as discussed in \cref{sec:DP}. Consequently, we challenge this assumption and modify the aforementioned  threat model to accommodate an adversary that is allowed to poison the training data of the owners it has control over. We also assume that the final trained model remains secret-shared among the outsourced servers to prevent additional leakage about the training data from the ML model~\cite{carlini2021}.


%differs  from our threat model. The main difference is in the power of the adversary $\Adv$ over the corrupted data owners. %Adversary $\Adv'$ is allowed to corrupt up to $m-1$ out of $m$ data owners, giving it more power (in terms corruption amount) than the adversary $\Adv$ in our setting. However, there is a massive limitation to the power of $\Adv'$ in terms control over each corrupted data owner: $\Adv'$ does not tamper with the training data of the owners it has corrupted. 
%Concretely,  in previous frameworks $\Adv$ could only observe (not modify) the training data of the corrupted owner and the final trained model returned to the owner.  In our threat model, we challenge this assumption and modify our threat model to accommodate an adversary that poisons the training data of the owners it has control over. We also assume that the final trained model remains secret-shared among the outsourced servers to prevent additional leakage about the training data from the ML model~\cite{carlini2021}.



%\noindent
%\newline
%{\bf Our Adversarial Model:}
%We first describe the role of  adversary $\Adv$ with respect to poisoning followed by its role in the SOC setting. Given $\Adv$ corrupts $t$ out $m$ data owners and $T$ out of $N$ servers, the role of $\Adv$ is as follows:
%\newline

%\begin{itemize}

%\item[--] 
\smallskip
%\noindent
\myparagraph{Poisoning Adversary} Existing threat models for training ML models privately assume that the local datasets contributed towards training  are not under the control of the adversary. However, data poisoning attacks have been shown to be a real threat when ML models are  trained on crowdsourced data or data coming from untrusted sources~\cite{BNL12,GBDPLR17,JOBLR18}. Data poisoning becomes a particularly relevant risk in PPML systems, in which data owners contribute their own datasets for training a joint ML model. Additionally, the datasets are secret shared among the servers participating in the MPC, and potential poisoned samples (such as backdoored data) cannot be easily detected by the servers running the MPC protocol.

To account for this attack vector, we define a poisoning adversary $\Ap$  that can  poison  a subset of local datasets of size at most $t <m$. We call the data owners with poisoned data as {\em poisoned owners}, and we assume that the adversary can coordinate with the poisoned owners to achieve a certain adversarial goal. For example, the adversary can mount a backdoor attack, by selecting a backdoor pattern and poison the datasets under its control with the particular backdoor pattern. 

%The impact of the attack could be amplified when multiple owners have poisoned data and we provide bounds on the level of poisoning tolerated by our designed framework.


% but we will show that in many instances a single poisoned owner by itself can mount a successful poisoning attack. We will also provide bounds on the level of poisoning tolerated by our designed framework.

{\em Poisoning Robustness:} We consider an ML model to be robust against a poisoning adversary $\Ap$, who poisons the datasets of $t$ out of $m$ owners, if it generates correct class predictions on new samples with high probability. We provide bounds on the level of poisoning tolerated by our designed framework to ensure robustness.



%Robustness informally means that the  model trained under the influence of a poisoned dataset still predicts the correct class label with a high probability.

%$\Ap$ incentivizes  these owners to  manipulate their training datasets in order to achieve a certain adversarial goal. We call such data owners as {\em `poisoned owners'}. The adversary can only control a small subset of such owners and we  later provide bounds for the level of poisoning tolerated. Additionally, the set of poisoned owners  are aware of the underlying algorithm used to train the model and can collude together to poison their dataset in order to introduce a desired characteristic in the learned parameters of the model.


\smallskip
%\noindent 
\myparagraph{Our Adversary} We now define a new adversary $\Apsc$  for our threat model (Figure~\ref{fig:AS}) that corrupts servers in the MPC and poisons the owners datasets:  
\begin{myitemize}
	\smallskip
	\item[--] $\Apsc$ plays the role of $\Ap$ and poisons $t$ out of $m$ data owners that secret share their training data to the outsourced servers.
	\item[--] $\Apsc$ plays the role of $\Asoc$ and corrupts $T$ out $N$ servers taking part in the MPC computation.
\end{myitemize}

\smallskip
Note that the poisoned owners that $\Apsc$ controls do not interfere in the execution of the MPC protocols after secret-sharing their data and also do not influence the honest owners. Additionally, to measure the attack success of the  poisoning attacks, adversary $\Ap$ needs query access to the trained model (inside the MPC)  at test time. To replicate this we let $\Apsc$ use its poisoned data owners from the training phase to query the  final trained model  at test time.

%Figure~\ref{fig:AS} provides a visual representation of our threat model. 

%$\Apsc$ plays the role of $\Ap$ and  fraction of owners that are used to poison the training data and a subset of servers that participate in the execution of the MPC protocols.

%As a whole, $\Adv$ is able to control a fraction of owners that are used to poison the training data and a subset of servers that participate in the execution of the MPC protocols. 


%$\Adv$ incentivizes the  owners it has corrupted to  poison their training datasets in order to achieve a certain adversarial goal. We call such data owners as {\em `poisoned owners'}. The adversary can only control a small subset of such owners and we  later provide bounds for the level of corruption tolerated. Additionally, the set of poisoned owners  are aware of the underlying algorithm used to train $\fm$ and can collude together to poison their dataset in order to introduce a desired characteristic in the learned parameters of $\fm$. For example, the poisoned owners can decide on a backdoor pattern and target class to mount a backdoor attack. Note that these poisoning attacks mounted by the poisoned owners do not break the privacy guarantees of the MPC protocols in the SOC setting, but instead influence the underlying trained model $\fm$ to achieve the attacker's poisoning objective. %Thus, the security definition of MPC alone does not prevent against these poisoning attacks.%\newline


%This is a rational assumption, for e.g, consider the case where a third party seller bribes users to give higher ratings to his/her product on an e-commerce website. Though a subset of users are compromised the total number of users are much higher resulting in a majority of honest users. Additionally, the set of corrupt owners $U_p$ are aware of the underlying algorithm used to train $\fm$ and can collude together to poison $\fd_p$ in order to introduce a desired characteristic in the learned parameters of $\fm$. Note that, these poisoning attacks carried out by the corrupt owners do not break the privacy guarantees of the MPC protocols carried out by the servers in the SOC setting, but instead influences the underlying trained model $\fm$ to achieve it's poisoning objective. 

%\smallskip
%{\em Role in  SOC paradigm:}  Once a subset of the  training data is poisoned, $\Adv$ plays the role of the adversary in the SOC paradigm. The exact values of $N$ and $T$ are dependent on the  MPC protocols that are used for training the model $\fm$. For instance, we experiment with two-party, three-party, and four-party protocols with one adversarial server. Along with the number of corruptions, the behavior of the adversary can also be divided into two main types: i) \emph{Semi-honest adversary}: Adversary follows the described protocol, but tries to derive additional information from the messages received from other parties during the protocol; ii) \emph{Malicious adversary}: Adversary has the ability to arbitrarily deviate during the execution of the protocol. For the purpose of our security proofs, we assume the adversary to be semi-honest in nature, but our approach can be extended to malicious adversaries. Fig. \ref{fig:AS} provides a representation of our threat model.


\smallskip
%\noindent
\myparagraph{Functionality  $\FpTrain$} Based on our newly introduced threat  model, we construct a new functionality $\FpTrain$ in Figure 2 to accommodate poisoned data. 

\begin{systembox}{$\FpTrain$}{Ideal Functionality for ML training with data poisoning}{func:pml}   
	\label{fig:ideal_func}
	
	\algoHead{Input:} $\FpTrain$ receives secret-shares of $\ld_i$ and $a_i$ from each owner $\usr_i$, where $\ld_i$ is a dataset and  $a_i$  an auxiliary input.
	
	
	\algoHead{Computation: } On receiving inputs from the owners, $\FpTrain$ computes $ O = f(\ld_1, . . . , \ld_m,a_1, \ldots,a_m)$, where $f$ and $O$ denotes the training algorithm and the output of the algorithm respectively.
	
	%	to server $S_i$, where $z_i$ denotes a secret-share of the trained model in appropriate format.
	
	\algoHead{Output:} $\FpTrain$ constructs secret-shares of $O$ and sends the appropriate shares to the servers.
	
	
	%	\algoHead{Parameters:}  A set $C = \{\usr_1,\ldots,\usr_m\}$ of data owners, where each owner $\usr_i$ posses:  dataset $\ld_i$ and an auxiliary input $a_i$. A set of outsourced servers  $S = \{S_1,\ldots,S_N\}$.
	
	%	 A set $U = \{\usr_1,\ldots,\usr_m\}$ of data owners with training datasets $\ld_1, \ldots, \ld_m$ respectively and a set $S = \{S_1,\ldots,S_N\}$ of outsourced servers.
	
	%	\smallskip
	%	\algoHead{Uploading Data:}  On input $\ld_i$ and $\fm_i$ from $\usr_i$, store $\ld_i$ and $\fm_i$ internally.
	
	%	\smallskip
	%	\algoHead{Computation}: On input training algorithm $f$ from one of the servers, compute $(z_1,\ldots, z_N)$ = $f(\ld_1, . . . , \ld_m,\fm_1, \ldots,\fm_m)$ and send  $z_i$ to server $S_i$, where $z_i$ denotes a secret-share of the robust trained model in appropriate format.
	
	%	\smallskip
	%	This step can be repeated multiple times with different algorithms.
\end{systembox}

%Figure~\ref{fig:ideal_pml} provides the details of our functionality.
%Note that, the $\FpTrain$  functionality we design is custom made based on our SafeNet framework and can vary depending on new frameworks that are  built on top of it.



\smallskip
%\noindent
\myparagraph{Security against $\Apsc$} A training protocol $\pistr$ is secure against adversary  $\Apsc$  if: (1)  $\pistr$ securely realizes functionality $\FpTrain$ based on Definition~\ref{def:mpc_sec}; and (2)  the   model trained inside the MPC provides poisoning robustness against data poisoning attacks.

Intuitively, the security definition ensures that $\Apsc$ learns no information about the honest owners' inputs when $T$ out of $N$ servers are controlled by the adversary, while the  trained model provides poisoning robustness  against a subset of $t$ out of $m$ poisoned owners. 

%\commentH{I personally think we need to have some sort of informal definition for security against poisoning. So that we can say SafeNet works well in our new threat model and provides security against adversary $\Apsc$}

%We provide details of the  local model, the robust training algorithm and the structure of the final trained model later in \cref{sec:SNoverview}. We define security using the ideal world-real world paradigm and provide a brief overview of the same in \cref{sec:SecDef}.


%but note that our approach can be extended for the case of a malicious adversary as well (assuming the underlying MPC framework supports malicious adversaries). 



%When viewed through an adversarial lens, this is an impractical assumption given the wide range of data poisoning attacks that already exist in the literature.


%Though $\Adv$ controls both the corrupt owners and the servers, we assign them different color codes in order to distinguish their roles in the threat model.

%are used to derive any additional information about other owners inputs

%\end{itemize}

%We consider a set of users $U = \{\usr_1,\ldots,\usr_m\}$ who want to train a joint machine learning model $\fm'$ on their combined datasets $\fd$. The users secret-share their respective datasets to a set of  outsourced servers that privately train $\fm'$ on $\fd$. We assume  only a small fraction out of the total participating users to be corrupt. These corrupt users are incentivized to poison the training dataset in order to achieve a certain adversarial objective.  

%This is a rational assumption, for e.g, consider the case where a third party seller bribes users to give higher ratings to his/her product on an e-commerce website. Though a subset of users are compromised the total number of users are much higher resulting in a majority of honest users. Additionally, all the corrupt users know the underlying training algorithm and can collude together to poison the training data accordingly. 
%All participating  users secret-share their datasets to a set of outsourced servers for training.

%\smallskip
%{\em MPC Framework: } We operate in the outsourced computation setting, where the inputs are secret-shared to a set of servers that perform the MPC computation. In our case, the input data for the training phase is collected from the participating users in secret-shared format, while the output is a trained model in secret-shared format among the servers.

% Our proposed defense approach is generalizable for any machine learning model and MPC framework that are equipped with the necessary MPC protocols to execute the building blocks of our defense framework. We present our protocols by invoking ideal functionalities for the corresponding building blocks. For purpose of completeness and simplicity, we assume the adversary to be semi-honest in nature; but note that it is easily extendable for the case of a malicious adversary. 
% for the purposes of evaluation we assume a three server setting with the majority of servers being honest, and that the inputs to the computation are provided in a secret-shared format.

%\begin{comment}

%\begin{comment }

%\end{comment }
%\end{comment}


==> algo.tex <==
\section{Using Ensembles in MPC}

In this section, we first describe the adversarial model considered in state-of-the-art privacy preserving ML training frameworks, and extend the model to allow the adversary to poison the training data of a subset of owners. We then discuss how to instantiate an ensemble in MPC, and prove that this protocol is robust to a variety of adversarial ML attacks. We then discuss a number of useful extensions to the protocol. Finally, we compare our protocol and extensions to existing techniques which take advantage of ensembles for their adversarial ML properties.

\subsection{Threat Model} \label{sec:threat_model}

{
	\begin{figure}[t ]
		\vspace{-1.5mm}	
		\begin{tikzpicture}[node distance= 0.7cm]
			\node(maldo1)[maldo]{ \footnotesize $\usr_1$ };
			%\node(maldo2)[maldo, below of=maldo1]{Data owner 2};
			\node(maldoi-1)[maldo, below of=maldo1]{\footnotesize $\usr_t$ };
			\node(hdoi)[hdo, below of=maldoi-1]{\footnotesize $\usr_{t+1}$ };
			\node(hdom)[hdo, below of=hdoi]{\footnotesize $\usr_m$ };
			
			\node(mals1)[malserver, right of = maldo1, xshift=4.6cm, yshift = -0.3cm]{\footnotesize S$_1$};
			
			\node(mals2)[malserver, right of = mals1, yshift = -0.8cm]{\footnotesize S$_2$};
			
			\node(malsT)[malserver, below  of = mals1, yshift = -1.0cm]{ \footnotesize S$_{\scaleto{T}{3pt}}$};
			
			\node(hsT1)[hserver, left  of = malsT, xshift = -0.4cm]{S$_{\footnotesize \scaleto{T+1}{3pt}}$};
			
			\node(hsN)[hserver, xshift = -0.4cm , left of = mals1]{S$_{\footnotesize \scaleto{N}{3pt}}$};
			
			\node(hsN1)[hserver, yshift = -0.8cm , left of = hsN]{S$_{\footnotesize \scaleto{N-1}{3pt}}$};
			
			\node(soc)[soc, left of = hsN, label= {\footnotesize SOC Paradigm}, xshift = 1.25cm, yshift = -0.85cm]{};
			
			\node(nota)[nota, below of = soc, xshift = - 2.1cm, yshift = -1.1cm]{};
			
			\node(mdnota)[mdnota, label = right: {\footnotesize Poisoned}, left of = nota, xshift = -2.3cm]{};
			\node(msnota)[msnota, right of = mdnota, label = right: {\footnotesize Corrupted}, xshift = 1.78cm]{};
			\node(hnota)[hnota, right of = msnota,label = right: {\footnotesize Honest}, xshift = 1.8cm]{};
			
			\path (maldo1) -- node[auto=false]{\ldots} (maldoi-1);
			%\path (maldoi-1) -- node[auto=false]{\ldots} (hdoi);
			\path (hdoi) -- node[auto=false]{\ldots} (hdom);
			\path (hdoi) -- node[auto=false]{\ldots} (hdom);
			
			\path[draw, densely dotted,  bend left] (mals2) edge (malsT);
			\path[draw, densely dotted,  bend left] (hsT1) edge (hsN1);
			
			\draw[sarrow](mals1) -- (mals2);
			\draw[sarrow](mals1) -- (malsT);
			\draw[sarrow](mals1) -- (hsT1);
			\draw[sarrow](mals1) -- (hsN1);
			\draw[sarrow](mals1) -- (hsN);
			
			\draw[sarrow](mals2) -- (malsT);
			\draw[sarrow](mals2) -- (hsT1);
			\draw[sarrow](mals2) -- (hsN1);
			\draw[sarrow](mals2) -- (hsN);
			
			\draw[sarrow](malsT) -- (hsT1);
			\draw[sarrow](malsT) -- (hsN1);
			\draw[sarrow](malsT) -- (hsN);
			
			\draw[sarrow](hsT1) -- (hsN1);
			\draw[sarrow](hsT1) -- (hsN);
			
			\draw[sarrow](hsN1) -- (hsN);
			
			\draw[darrow](maldo1) -- (soc);
			\draw[darrow](maldoi-1) -- (soc);
			\draw[darrow](hdoi) -- (soc);
			\draw[darrow](hdom) -- (soc);
		\end{tikzpicture}
		\caption{Threat model considered in our setting. The adversary $\Apsc$ can poison at most $t$ out of $m$ data owners and corrupt at most $T$ out of $N$ servers participating in the MPC computation. $\usr_i$ and $\srvr_j$ denote the $i^{th}$ data owner and $j^{th}$ server respectively.}
		\label{fig:AS}
		\vspace{-1.5mm}
\end{figure}}



\myparagraph{Setup} We consider a set of $m$ data owners $C= \cup_{k=1}^{m} \usr_k$ who wish to train a joint machine learning model $\fm$ on their combined dataset $\fd =  \cup_{k=1}^{m} \ld_k$. We adopt the Secure Outsourced Computation (SOC) paradigm~\cite{MohasselZ17, MR18, WaghGC18, PS20, BCPS20, RRKCGRS20, WTBKMR21, AEV21, DEK20, DEK21} for training model $\fm$ privately, where the owners secret-share their respective datasets to a set of  outsourced servers, who enact the role of mutually distrusting  parties in the MPC and execute the necessary protocols to train $\fm$. The final output after execution of these protocols is a trained model in secret-shared format among the servers.  
A single training/testing sample is expressed as $(\ssample_i, \slbl_i)$, where $\ssample_i$ is the input feature vector and $\slbl_i$ is its corresponding true label or class. We use $\ld_k = (\dataset_{\sss{k}}, \lbl_{\sss{k}})$ to denote dataset of data owner $\usr_k$ participating in the training process. Matrix $\dataset_{\sss{k}}$ denotes a feature matrix where the number of rows represent the total training samples possessed by $\usr_k$ and $\lbl_{\sss{k}}$ denotes the corresponding vector of true labels.

\smallskip
%\noindent
\myparagraph{Adversary in the SOC} Given  a set $S = \{\srvr_1,\ldots,\srvr_N\}$ of outsourced servers, we define an adversary $\Asoc$,  similar to prior work~\cite{MohasselZ17, MR18, RRKCGRS20, WTBKMR21, AEV21, DEK21}.  $\Asoc$ can statically corrupt a  subset $S_T \subset S$ of servers of size at most $T<N$. The exact values of $N$ and $T$ are dependent on the  MPC protocols  used for training the ML model privately. For instance, we experiment with two-party, three-party, and four-party protocols with one corrupt server. MPC defines two main adversaries: i) \emph{Semi-honest}: Adversary follows the described protocol, but tries to derive additional information from the messages received from other parties during the protocol; ii) \emph{Malicious}: Adversary has the ability to arbitrarily deviate during the execution of the protocol. For our security proofs, we assume the adversary to be semi-honest, but our approach can be extended to malicious adversaries.

\smallskip
%\noindent
\myparagraph{Security Definition} MPC security is defined using the real world - ideal world paradigm~\cite{C00}.
In the real world, parties participating in the MPC interact during the execution of a protocol $\pi$ in presence of an adversary $\Adv$. Let $\mathsf{REAL}[\mathbb{Z}, \Adv, \pi, \lambda]$ denote the output of the environment $\mathbb{Z}$ when interacting with $\Adv$ and the honest parties, who execute $\pi$ on security parameter $\lambda$. This interaction is called the real-world interaction. Effectively, $\mathsf{REAL}$ is a function of the inputs/outputs and messages sent/received during the protocol. In the ideal world, the parties simply forward their inputs to a trusted functionality $\mathcal{F}$ and forward the functionality's response to the environment.
Let $\mathsf{IDEAL}[\mathbb{Z}, \Sim, \mathcal{F}, \lambda]$ denote the output of the environment $\mathbb{Z}$ when interacting with adversary $\Sim$ and honest parties who run the  protocol in presence of $\mathcal{F}$ with security parameter $\lambda$. The security definition states that the views of the adversary in the real and ideal world are indistinguishable: 

\begin{definition} \label{def:mpc_sec}
	A  protocol $\pi$ securely realizes  functionality $\mathcal{F}$   if for all environments $\mathbb{Z}$ and any adversary of type $\Asoc$, which  corrupts a subset $S_T$ of servers of size at most $T < N$ in the real world, then there exists a simulator $\Sim$ attacking the ideal world, such that $\mathsf{IDEAL}[\mathbb{Z}, \Sim, \mathcal{F}, \lambda] \approx \mathsf{REAL}[\mathbb{Z}, \Asoc, \pi, \lambda]$.
\end{definition}


\begin{comment}
\begin{systembox}{$\FTrain$}{Ideal Functionality for ML training}{func:ml}   \label{fig:ideal_ml}
	\algoHead{Parameters:} A set $U = \{\usr_1,\ldots,\usr_m\}$ of data owners with training datasets $\ld_1, \ldots, \ld_m$ respectively and a set $S = \{S_1,\ldots,S_N\}$ of outsourced servers.
	
	\smallskip
	\algoHead{Uploading Data:}  On input $\ld_i$ from $\usr_i$, store $\ld_i$ internally.
	
	\smallskip
	\algoHead{Computation}: On input ML training algorithm $f$ from one of the servers, compute $(z_1,\ldots, z_N)$ = $f(\ld_1, . . . , \ld_m)$ and send  $z_i$ to server $S_i$, where $z_i$ denotes a secret-share of the trained model in appropriate format.
	
	\smallskip
\end{systembox}
\end{comment}

\smallskip
\myparagraph{Poisoning Adversary} Existing threat models for training ML models privately assume that the local datasets contributed towards training  are not under the control of the adversary. However, data poisoning attacks have been shown to be a real threat when ML models are  trained on crowdsourced data or data coming from untrusted sources~\cite{BNL12,GBDPLR17,JOBLR18}. Data poisoning becomes a particularly relevant risk in PPML systems, in which data owners contribute their own datasets for training a joint ML model. Additionally, the datasets are secret shared among the servers participating in the MPC, and potential poisoned samples (such as backdoored data) cannot be easily detected by the servers running the MPC protocol.

To account for this attack vector, we define a poisoning adversary $\Ap$  that can  poison  a subset of local datasets of size at most $t <m$. We call the data owners with poisoned data as {\em poisoned owners}, and we assume that the adversary can coordinate with the poisoned owners to achieve a certain adversarial goal. For example, the adversary can mount a backdoor attack, by selecting a backdoor pattern and poison the datasets under its control with the particular backdoor pattern. 


{\em Poisoning Robustness:} We consider an ML model to be robust against a poisoning adversary $\Ap$, who poisons the datasets of $t$ out of $m$ owners, if it generates correct class predictions on new samples with high probability. We provide bounds on the level of poisoning tolerated by our designed framework to ensure robustness.

\smallskip
\myparagraph{Privacy Adversary} While MPC guarantees no privacy leakage from the protocol, it makes no guarantees about privacy leakage from the output of the model. This has motivated the combination of differential privacy guarantees with MPC algorithms, to protect both the transcript of the protocol as well as the output of the protocol. For this reason, we consider also adversaries seeking to learn information about data owners' local datasets, in both membership inference and property inference attacks. This adversary need not be semi-honest: prior work has shown that an adversary capable of actively manipulating training with poisoning data is also capable of improved privacy leakage~\cite{}. To do so, the adversary makes queries to the output of the protocol at test time.

{\em Differential Privacy:} Differential privacy is a well-known notion of data privacy which applies to the output of a computation on a database. Differential privacy also provides (weak) robustness to inference attacks against groups, via its group privacy property.

\smallskip
\myparagraph{Our Adversary} We now define a new adversary $\Apsc$  for our threat model (Figure~\ref{fig:AS}) that corrupts servers in the MPC, poisons the owners' datasets, and observes the output of the computation:  
\begin{myitemize}
	\smallskip
	\item[--] $\Apsc$ plays the role of $\Ap$ and poisons $t$ out of $m$ data owners that secret share their training data to the outsourced servers.
	\item[--] $\Apsc$ plays the role of $\Asoc$ and corrupts $T$ out $N$ servers taking part in the MPC computation.
	\item[--] $\Apsc$ is capable of observing the output of the computation and wants to perform membership inference and property inference attacks on the training set of other models.

\end{myitemize}

\smallskip
Note that the poisoned owners that $\Apsc$ controls do not interfere in the execution of the MPC protocols after secret-sharing their data and also do not influence the honest owners. Additionally, to measure the attack success of the  poisoning attacks, adversary $\Ap$ needs query access to the trained model (inside the MPC) at test time. To replicate this we let $\Apsc$ use its poisoned data owners from the training phase to query the  final trained model  at test time.

\smallskip
\myparagraph{Functionality  $\FpTrain$} Based on our newly introduced threat  model, we construct a new functionality $\FpTrain$ in Figure 2 to accommodate poisoned data. 

\begin{systembox}{$\FpTrain$}{Ideal Functionality for ML training with data poisoning}{func:pml}   
	\label{fig:ideal_func}
	
	\algoHead{Input:} $\FpTrain$ receives secret-shares of $\ld_i$ and $a_i$ from each owner $\usr_i$, where $\ld_i$ is a dataset and  $a_i$  an auxiliary input.
	
	\algoHead{Computation: } On receiving inputs from the owners, $\FpTrain$ computes $ O = f(\ld_1, . . . , \ld_m,a_1, \ldots,a_m)$, where $f$ and $O$ denotes the training algorithm and the output of the algorithm respectively.
	
	\algoHead{Output:} $\FpTrain$ constructs secret-shares of $O$ and sends the appropriate shares to the servers.

\end{systembox}

\smallskip
\myparagraph{Security against $\Apsc$} A training protocol $\pistr$ is secure against adversary  $\Apsc$  if: (1)  $\pistr$ securely realizes functionality $\FpTrain$ based on Definition~\ref{def:mpc_sec}; and (2)  the   model trained inside the MPC provides poisoning robustness against data poisoning attacks.

Intuitively, the security definition ensures that $\Apsc$ learns no information about the honest owners' inputs when $T$ out of $N$ servers are controlled by the adversary, while the  trained model provides poisoning robustness  against a subset of $t$ out of $m$ poisoned owners. 


\subsection{Setting Up an Ensemble}\label{sec:SNoverview}
%\begin{comment}
\begin{figure*}[t] 
	%	\vspace{-3mm}
	%\centering
	\includegraphics[scale=0.3]{SafeNet_Overview.pdf}
	\caption{Overview of the Training and Testing phases of the \safenet Framework.}
	\label{fig:EF}
	%	\vspace{-4mm}
\end{figure*}
%\end{comment}


Given our threat model in Figure~\ref{fig:AS}, existing PPML  frameworks provide security against an $\Asoc$ adversary, but they are not designed to handle an  adversary of type  $\Apsc$. We show experimentally in Section~\ref{sec:exp} that PPML frameworks for private training are susceptible to data poisoning attacks.  While it would be possible to remedy this by implementing specific poisoning defenses (see Section~\ref{sec: otherDefenses} for a discussion of these approaches), we instead show that it is possible to take advantage of the bounded poisoning capability of $\Apsc$ to design a more general and efficient defense. Intuitively, existing approaches train a single model on all local datasets combined, causing the model's training set to have a large fraction of poisoned data ($t/m$), which is difficult to defend against. Instead, we design SafeNet, a new framework which uses ensemble models to realize our threat model and provide security against $\Apsc$. In addition to successfully mitigating data poisoning attacks, SafeNet provides more efficient training than existing PPML and comparable prediction accuracy.


 %Existing privacy-preserving ML training frameworks are unequipped with the necessary tools to mitigate data poisoning attacks introduced by the poisoned data owners. In order to address this issue, we propose an alternate training method which not only gives prediction accuracy comparable to the traditional model and efficient training, but is also able to successfully mitigate data poisoning attacks.  

Figure~\ref{fig:EF} provides an overview of the training and testing phases of SafeNet. \safenet trains an ensemble $E$ of multiple models in protocol $\pistr$, where each model $\fm_k \in E$ is trained locally by the data owner $\usr_k$ on their dataset. This partitioning prevents poisoned data from contributing to more than $t$ local models. Each data owner samples a local validation dataset and trains the local model $\fm_k$ on the remaining data. The local models and validation datasets are secret shared to the outsourced servers. We note that this permits arbitrarily corrupted models, and poisoned validation datasets, but SafeNet's structure still allows it to tolerate these corruptions. In the protocol running inside the MPC, the servers jointly implement a filtering stage for identifying models with low accuracy on the combined validation data  (below a threshold $\phi$) and excluding them from the ensemble. The output of training is a secret share of each model in the trained ensemble $E$. Note that exclusion in this case does not mean explicitly removing the model from the ensemble, but, instead, not including the model's prediction in the testing voting procedure. Later in Section  \ref{sec:sectrain}, we show a way to realize the filtering stage without revealing which models is excluded from the final ensemble.

%Towards this goal, the servers compute the validation accuracy on the global validation set $\CV$ and remove models with accuracy lower than a fixed threshold $\phi$. 

In the prediction phase, SafeNet implements protocol $\piPred$, which generates the prediction $y_k$ of each shared model $\fm_k$ on test input $x$ inside the MPC. The servers  jointly perform majority voting to determine the most common predicted class $y$ on input $x$, using only the models which pass the filtering stage.

%In addition, each data owner contributes a small fraction of its dataset to construct a common validation dataset, which we use to compute accuracy for each ensemble model. We use this phase in order to filter models from the ensemble that have low accuracy on the common validation dataset. 
%We will show that this filtering procedure prevents poisoning availability attacks.
% The remaining models in the ensemble are secret shared among the servers participating in the SOC protocol. 
%The filtered ensemble is then used to generate a prediction where the servers run an MPC protocol to perform majority voting over the individual models predictions.  

Our \safenet protocol leverages our threat model, which assumes that only a set of at most $t$ out of $m$ data owners are poisoned. This ensures that an adversary only influences a limited set of models in the ensemble, while existing training protocols would train a single poisoned global model. We provide bounds for the exact number of poisoned owners $t$ supported by our ensemble in Theorem~\ref{thm:LB}. Interestingly, the bound depends on the number of data owners $m$, and the maximum error made by a clean model in the ensemble.  The same theorem also lower bounds the probability that the ensemble predicts correctly under data poisoning performed by the $t$ poisoned owners, and we validate experimentally that, indeed, \safenet provides resilience to stealthy data poisoning attacks, such as backdoor and targeted attacks. Another advantage of \safenet is that the training time to execute the MPC protocols in the SOC setting is drastically reduced as each $\fm_k \in E$ can be trained locally by the respective owner. 
%
We detail below the algorithms for training and prediction in SafeNet. 

%The only protocols implemented in the MPC are: (1) Ensemble Filtering; and (2) \safenet prediction, which we detail below.

%Concretely, our approach is to build an ensemble $E$ where each model $\fm_k \in E$ is trained on the dataset $ \ld_k \in \fd$ possessed by the data owner $\usr_k$. This constructed $E$ replaces $\fm$, which was earlier trained over the combined dataset $\fd$. The advantages of our approach are two fold:


%For simplicity, we describe the working of our SafeNet framework as a two step process:
%\begin{itemize}
%	\item [--] The first step computes the {\OB} accuracy of each model which  help us to differentiate between the behavior of an honest from a corrupt owner.

%	\item[--] The second step compares each model's {\OB} accuracy with a pre-agreed threshold to remove poisoned or poorly performing models from $E$.
%\end{itemize}



\begin{comment}
\begin{figure}[h!]
\caption{Schematic representation of SafeNet Framework}
\label{fig:EF}

\vspace{2mm}
\begin{tikzpicture}[node distance= 1cm]

\node(maldo)[draw, text centered, text width=2.7cm,fill=orange!70, font = \small, xshift = -4cm] {Corrupt owners \\ Dataset and Models};

\node(hdo)[draw, text centered, text width=2.7cm,right of  = maldo, font = \small, xshift = 4.2cm,fill=cyan!55] {Honest owners \\ Dataset and Models};

\node(uoob)[draw, text centered, rounded corners, text width=2.7cm,below of  = maldo, font = \small, xshift = 2.6cm,yshift = -0.4cm, fill=white!60] {$\OB$ Accuracy};

\node(tc)[draw, text centered,rounded corners, text width=2.7cm,font = \small, below of  = uoob, fill=white!60] {Threshold Comparison};

\node(fe)[draw, text centered, rounded corners, text width=2.7cm,below of  = tc, font = \small, fill=white!60] {Final Ensemble};

\node(soc)[soc,  minimum height=2.8cm, above of = uoob, label= {\footnotesize Ensemble Filtering}, yshift = -2cm]{};

\path[draw,-latex,  bend right] (maldo) edge (uoob);
\path[draw,-latex,  bend left] (hdo) edge (uoob);
\path[draw,-latex] (uoob) edge (tc);
\path[draw,-latex] (tc) edge (fe);
\end{tikzpicture}

\end{figure}
\end{comment}


\subsection{\safenet Training} \label{sec:train}

To train the ensemble in SafeNet, we show our proposed ensemble method in Algorithm 1. We  discuss the realization in MPC  later in Section~\ref{sec:mpc_inst}. Each owner $\usr_k$ separates out a subset of its training dataset $\cv{k} \in \ld_k$ and then trains its model $\fm_k$ on the remaining dataset $\ld_k \setminus \cv{k}$. The trained model $\fm_k$ and validation dataset $\cv{k}$ is then secret-shared to the servers. The combined validation dataset is denoted as $\CV = \bigcup\limits_{i=1}^{m} \cv{i}$. We assume that all users contribute equal-size validation sets to $\CV$. During the filtering stage inside the MPC, the validation accuracy $\valacc$ of each model is jointly computed on $\CV$. If the resulting accuracy for a model is below threshold $\threshold$, the model is excluded from the  ensemble. 

%\newcommand{\pistr}{\ensuremath{\Pi_\mathsf{str}}}

The  filtering step is used to separate the models with low accuracy, either contributed by a poisoned owner, or by an owner holding non-representative data for the prediction task.
%prevents against an adversary contributing a low-accuracy model (e.g., a model trained on random labels of the data), or against an owner holding a non-representative dataset for the learning task. 
  Under the assumption that the majority of owners are honest, it follows that the majority of validation samples are correct. If  $\usr_k$ is honest, then the corresponding $\fm_k$ should have a high validation accuracy on $\CV$, as the corresponding predicted outputs would most likely agree with the samples in $\CV$. In contrast, the predictions by a poisoned model $\fm_k$ will likely not match the samples in $\CV$.  In Section~\ref{sec:bounds}, we compute a lower bound on the size of the validation dataset as a function of  the number of poisoned owners $t$ and filtering threshold $\threshold$, such that all clean models pass the filtering stage with high probability even when a subset of the cross-validation dataset $\CV$ is poisoned. 

Given protocol $\pistr$ that securely realizes Algorithm 1 inside the MPC (which we will define later in Section~\ref{sec:mpc_inst}), we argue security as follows:

\begin{restatable}{theorem}{SPtrain} \label{thm:SNtrain}
Protocol $\pistr$ is secure against  adversary $\Apsc$ who poisons $t$ out of $m$ data owners and  corrupts $T$ out of $N$ servers.
\end{restatable}

\noindent
The proof of the theorem will be given in Appendix~\ref{app:secproof} after we introduce all the details of MPC instantiation and how  protocol $\pistr$ securely realizes $\FpTrain$ in Section \ref{sec:sectrain}. 

%Note that, the inputs to $\FpTrain$ with respect to each owner $\usr_i$ would be dataset $D_i = \cv{i}$ and auxiliary input $a_i = \fm_i$.

%This way, we can set the threshold value $\threshold$ according to the number of poisoned owners $t$ and the expected worst-case error by the clean models. We discuss the impact of choice of $\threshold$ on ensemble filtering stage and later in \cref{sec:fashion_nn}.

%\commentH{Add theorem here stating safenet training securely realizes $\FpTrain$}.


%The "$\OB$ (Owner-Out-Of-Bag)" accuracy for a given owner $\usr_k$ is calculated by computing the predictions of her/his trained model $\fm_k$ over a dataset $\fd_{ob}$, followed by comparing the predicted outputs to their respective true labels. 

%Thus, for each owner $\usr_k$, dataset $\fd_{ob}$ acts a cross-validation/$\OB$ dataset and  will have a $\OB$ accuracy associated with her/his model $\fm_k$. 
%The reason behind using $\OB$ accuracy as a parameter for selection is  based on the prior knowledge that the  $\fd_{ob}$ comprises of data samples from honest owners in majority. If  $\usr_k$ is honest then the corresponding $\fm_k$, when tested against $\fd_{ob}$ should have a high $\OB$ accuracy as the corresponding predicted outputs would probably agree with most of the true labels associated with the samples in $\fd_{ob}$, as majority of the samples in $\fd_{ob}$ constitute the honest owners $\OB$ dataset. A similar argument can be made for a corrupt $\usr_k$ where her/his predicted outputs will mismatch with the labels associated to the samples in $\fd_{ob}$. 

%This strategy works against certain types of attacks (for eg. availability attacks)  where the goal of the adversary is to decrease the accuracy of the ensemble $E$ . Our filtering strategy will remove such models as each corrupt owner can reduce the accuracy of $E$, only by causing it's own model to perform poorly which will highly likely have its $\OB$ accuracy less than a sepcified threshold $T$.
%
% Similarly, if $\usr_k$ is corrupt, $\pred_{\sss{\ld_i}}$ will most likely agree with the labels associated with the samples of other corrupt users but may have many mismatches with the labels associated to the samples submitted by the honest users (who are in majority). Thus on an average the u-OOB accuracy for a $\lm_i$ submitted by an honest user is likely to be more than the u-OOB accuracy for a $\lm_i$ of a corrupt user. We concretize our claims later in section \ref{sec:RPA}, where we observe the variation in u-OOB accuracy for an honest and corrupt user with change in pollution amount. 

%\begin{comment}


\begin{algorithm}[t]
	
	\caption*{{\bf Algorithm 1} SafeNet Training Algorithm} \label{alg:ensemblefiltering}
	\begin{algorithmic}
		
		%\smallskip
			\State Input: $m$ data owners, each owner $\usr_k$'s   dataset $\ld_k$. 	
		%		, owner-out-of-bag data  $\fd_{ob} = \bigcup\limits_{i=1}^{m} \ld^{ob}_i$ and threshold $T$.				
		%		ensemble of models $ E = \lbrace \fm_i \rbrace_{i=1}^{m}$
		%\smallskip
			 \Comment{\footnotesize Owner's local computation in plaintext format} 
			\State -- For $k \in [1,m]:$	
			\begin{itemize}
				\item[-] Separate out $\cv{k}$ from $\ld_k$. Train $\fm_k$ on $\ld_k \setminus \cv{k}$.
				\item[-] Secret-share $\cv{k}$ and $\fm_k$ to servers.
			\end{itemize}
		
		%\smallskip
%		\State Owners also secret-share a pre-agreed threshold $\threshold$ to the servers.
		
		%\smallskip
			\Comment{\footnotesize MPC computation in secret-shared format}
			\State -- Construct a common validation dataset $\CV = \cup_{i=1}^{m} \cv{i}$ and collect ensemble of models $ E = \lbrace \fm_i \rbrace_{i=1}^{m}$
		
			\State -- Initialize a vector $\valvec$ of zeros and of size $m$. 
		
		%\smallskip
			\State  -- For $k \in [1,m]:$ \Comment{\footnotesize Ensemble Filtering}
			\begin{itemize}
				\item[-] $\valacc_k = Accuracy(\fm_k, \CV)$ \Comment{\footnotesize Compute validation accuracy of $\fm_k$ over $\CV$. }
			
%			\item[-] $\textsc{Preds}_k = \fm_k(\fd_{ob})$  \Comment{Compute output predictions of $\fm_k$ over $\fd_{ob}$. }
			
			%\item[-] $\text{O}^3\text{B}_\text{k} = \frac{1}{\abs{\fd_{ob}}} \sum_{i=1}^{\abs{\fd_{ob}}}\mathbbm{1}[\textsc{Preds}^i_k == \text{y}^i_{\fd_{ob}}]$ \Comment{Compute $\OB$ accuracy of the model.}
			
				\item[-] If $\valacc_k> \threshold$: \Comment{\footnotesize Compare against threshold} 
				\begin{itemize}
					\item[--] Set $\valvec_k = 1$   \Comment{\footnotesize Set $k^{th}$ position in $\valvec$ to 1} 
				
				%	\item[-] $ \textsc{Ensemble} = \textsc{Ensemble} \cup  \fm_i$   \Comment{add models in final ensemble if u-OOB accuracy greater than threshold}
				\end{itemize}			
			
			\end{itemize}
		%\smallskip
			\State \Return $E$ and $\valvec$
		\end{algorithmic}
%		\caption{SafeNet Training Algorithm}{}
\label{alg:train}
\end{algorithm} 


\begin{comment} 
\begin{algorithm}
\begin{algorithmic}

\State Input: number of data owners $m$, ensemble of models $ E = \lbrace \fm_i \rbrace_{i=1}^{m}$ , owner-out-of-bag data  $\fd_{ob} = \bigcup\limits_{i=1}^{m} \ld^{ob}_i$ and threshold $T$.
%\State $\textsc{Ensemble} = \{\}$

\State For $k \in [1,m]:$
\begin{itemize}
\item[-] $\textsc{Preds}_k = \fm_k(\fd_{ob})$  \Comment{Compute output predictions of $\fm_k$ over $\fd_{ob}$. }

\item[-] $\text{O}^3\text{B}_\text{k} = \frac{1}{\abs{\fd_{ob}}} \sum_{i=1}^{\abs{\fd_{ob}}} \textsc{Preds}^i_k == \text{y}^i_{\fd_{ob}}$ \Comment{Compute $\OB$ accuracy of the model.}

\item[-] If $\OB_k< T$: 
\begin{itemize}
\item[--] Remove $\fm_i$ from ensemble $E$.

%	\item[-] $ \textsc{Ensemble} = \textsc{Ensemble} \cup  \fm_i$   \Comment{add models in final ensemble if u-OOB accuracy greater than threshold}
\end{itemize}			

\end{itemize}


\State \Return $E$
\end{algorithmic}
\caption{SafeNet Training Algorithm \alina{I think this algorithm should start from input the datasets, Then we need to add training  models locally and construction of validation data.}}
\label{alg:ensemblefiltering}
\end{algorithm} 

\begin{algorithm}
\begin{algorithmic}

\State Input: number of model providers (data owners) $p$, number of models per provider $q$, set of models $ E = \lbrace \fm_i \rbrace_{i=0}^{qp-1}$ , combined data from model providers $\fd = \bigcup\limits_{k=1}^{p} \ld_k$ and threshold $T$.
%\State $\textsc{Ensemble} = \{\}$

\State For $k \in [p]:$
\begin{itemize}
\item[] For $i \in [(k-1)q, kq-1]:$
\begin{itemize}
\item[-] $\textsc{Preds}_i = \fm_i(\dataset_{\sss{\fd}} / \dataset_k)$

\item[-] If $\text{O}^3\text{B}~\textsc{(Preds}_i,~ \lbl_{\sss{\fd}} / \lbl_k) < T$: 
\begin{itemize}
\item[--] Remove $\fm_i$ from set $E$.

%	\item[-] $ \textsc{Ensemble} = \textsc{Ensemble} \cup  \fm_i$   \Comment{add models in final ensemble if u-OOB accuracy greater than threshold}
\end{itemize}			

\end{itemize}
\end{itemize}


\State \Return $E$
\end{algorithmic}
\caption{Ensemble Filtering Algorithm}
\label{alg:ensemblefiltering}
\end{algorithm}
\end{comment}


\input{RobustBounds}

\input{mpc_instantiation.tex}



==> algo_old.tex <==
\section{\safenet Framework}

\input{SecDef}

\input{SafenetDetails}

\input{RobustBounds}

\input{mpc_instantiation.tex}



==> last_reviews.tex <==
% \documentclass[conference]{IEEEtran}

% \pagestyle{plain}
% \begin{document}
\section*{Changes from previous submission}
\begin{enumerate}
    \item We made some additions that were not related to reviewer comments. We added transfer learning experiments on CIFAR-10, the first CIFAR-10 training setup we are aware of in MPC. We showed that SafeNet can be modified to satisfy differential privacy, and discussed how this modification can impact provable robustness guarantees. We add experiments on EMNIST, a non-iid federated learning benchmark dataset.
    
    \item Reviewer A has concerns about the novelty of the approach, as we do not design new MPC primitives, and other works have proposed using ensembles to defend against poisoning and privacy. In response to this comment, we added significant comparison to prior works (Section III-F). We also added new privacy analysis and added more extensions that support transfer learning and computationally restricted owners.
    
    \item Reviewer A suggested we compare to the PATE framework. We compared to this framework, and realized that our approach actually admits a much stronger privacy protection than is offered by PATE, user-level differential privacy! We also discuss the interaction between provable privacy and provable poisoning robustness.
    
    \item Reviewer A asked if we could use different thresholds for each user. This is possible, but we choose not to do this, as there is no clear reason to do so.
    
    \item Reviewer B asks if ensembling has higher accuracy than individual models. This is the main reason why ensembles are used in practice, even when trained on the exact same data! To address this, we added individual and SafeNet model accuracies to the paper in Section IV-D. SafeNet improves over individual model accuracies even in EMNIST, a benchmark non-iid ``cross-user" federated learning dataset, as seen in Section IV-D. However, for extreme non-iid settings, SafeNet's accuracy degrades as expected (see experiments from Appendix E-A). Fortunately, SafeNet being very cheap to run allows it to ``fail fast", and let these parties know that it is not applicable in their setting. We try to position SafeNet in this way - less as a ``all-around'' solution for PPML, and more as a quick, simple strategy that is easy to quickly test and has strong adversarial ML properties.
\end{enumerate}


\section*{NDSS 2023 - Reviewer A} Recommendation: 2. Leaning towards reject

\paragraph*{Writing quality} 4. Well-written

\paragraph*{Expertise}
3. Knowledgeable

\paragraph*{Summary}
This paper proposes SafeNet, a general framework for building ensemble (or a set of) models in secure multiparty computation (MPC) with robustness to (backdoor and targeted) poisoning attacks. Almost all the MPC frameworks for ML do not consider the robustness issue, i.e., they train a single model on all local datasets assuming these datasets are not corrupted by an adversary. To address it, SafeNet is proposed. In more detail, each data owner splits its dataset into a training subset and a validation subset (to be secretly shared among different parties for MPC). It then trains a model locally on its training subset. The model will be secretly shared among different parties/servers under the MPC paradigm: they first screen out local models with low accuracy using the combined validation set, then make predictions on the remaining models using majority voting under MPC.

Besides some theoretical bounds on e.g., the test accuracy and number of poisoned owners, the authors also conducted experiments on different models (such as logistic regression and deep neural networks) and four datasets.

\paragraph*{Strengths}
\begin{enumerate}
    \item Providing robustness (to data poisoning) in secure machine learning (ML) via MPC is vital and promising.
    \item Compared to a secure 4PC framework [26], SafeNet can effectively defend against backdoor attacks and obtain significant efficiency gain (e.g., 39x faster).
\end{enumerate}

\paragraph*{Weaknesses}
\begin{enumerate}
    \item The paper could be improved by better justifying its contribution. The current technical contribution appears to be limited given the existing ensemble models idea and MPC primitives. The idea is simple and effective, but not new. As pointed out by the authors in a short paragraph (Sect. II-C), model ensembles have been already used for defending against poisoning [9, 47] and protecting privacy [23]. Furthermore, SafeNet just makes black-box use of existing MPC primitives (and other ML primitives) in Sect. III-E (e.g., secret sharing) for instantiation in the MPC setting.
    \item The threat model is not that clear in terms of the MPC part. See C1.
\end{enumerate}

\paragraph*{Detailed Comments}
\begin{enumerate}
    \item The authors extend the original MPC security definition $A_{soc}$ to additionally cover the poisoning robustness $A_p$, leading to the security against an adversary $A^p_{soc}$ (see the left column in p4). For $A^p_{soc}$, the authors only focus on that it can poison "t out of n" data owners and corrupt "T out of N" servers, albeit $A_p$ is further restricted to the backdoor and targeted poisoning. However, $A_{soc}$ is unclear. In more detail, the servers are semi-honest vs. malicious? What are the malicious behaviors (if malicious security is considered)? Whether those malicious behaviors would affect the robustness? honest majority vs. dishonest majority?
    \item Another related framework of PATE [PSMRTE18] is can be discussed. In PATE, different teacher models are first trained on datasets. For aggregating models and predictions, PATE also adopts majority voting (in particular, on the noisy vote histograms for preserving privacy).
  [PSMRTE18] N. Papernot et al. Scalable Private Learning with PATE. ICLR'18.
  \item There is a global threshold $\phi$ (for all the data owners) set to screen out models with low accuracy. A natural question is that can such a threshold be adaptively set for each data owner?
  \item Minor issues and typos, e.g.:
  - too many notations spread throughout the paper, the authors could summarize them in a table.
  - right column of p6, "of x" where x should be in math mode.
\end{enumerate}


\paragraph*{Ethics} 3. No ethic issues


\section*{NDSS 2023 - Reviewer B} Recommendation: 2. Leaning towards reject

\paragraph*{Writing quality}
3. Adequate

\paragraph*{Reviewer expertise}
3. Knowledgeable

\paragraph*{Summary}
The paper proposes SafeNet, a framework for building machine learning model ensemble (based on voting) using  secure outsourced computation. Experiments on some benchmark datasets show the resilience of SafeNet to poisoning attacks.

\paragraph*{Strengths}
The paper is well motivated and the proposed approach is thoroughly described.
The experimental section and the discussion are also well done.

\paragraph*{Weaknesses}
The proposed approach is somewhat naive and I am not sure (from what I read in the paper) that in real scenarios it is effective and resilient as reported in the paper.

\paragraph*{Detailed Comments}
\begin{enumerate}
    \item My main concern about this work is related to the approach (SafeNet). As far as I understood, Safenet builds a majority voting ensemble where the single learners are trained (using SOC) on separate datasets (owned by the data owners). Then, using a validation set, models are kept in the ensemble iff are “good enough” (estimation based on a threshold). My concern is that the voting ensemble is not guaranteed to perform better than any single model used in the ensemble, especially if learned on different portions of the dataset. For sure, the ensemble can help reduce the variance. However, it must be shown that it is better than the single models, especially if the models are trained on a sufficiently large sample.
    \item Regarding the security aspects, some of the reported results seem too good to be true in the sense that the attack only works when at least half of the owners are poisoned (which in this case the attack has to work by definition). However, this behavior can happen if, and only if, there is total agreement on the correct label across the non-poisoned models. Indeed, in the TGT-Foot experiments, the rate of success against SafeNet is a bit higher (~20\%). Still, there is a good agreement between the models. In my opinion, this may happen if the task is very simple and data are iid distributed. In any case, what is missing in the experiments is how good are the single models (the ones built using the data of each single data owner). I suspect that, in the case of iid data distribution, each model performs as well as the ensemble, thus making the ensemble somewhat superfluous. This consideration is also supported by the results reported in Fig. 10. With no poisoning, the ensemble works precisely as the federated model, which is somewhat suspicious considering that the federated model is trained on all the data. As said, this behavior is reasonable only because data are iid, and hence the single models are working just fine. Maybe the authors should investigate this and add some considerations/justifications.
\end{enumerate}





Other minor issues:
* The authors mentioned that they split the dataset into 20 data owners for all dataset but Fashion. Why?
* Algorithms are badly formatted (e.g., Algorithm 1)
* In the proof of Theorem 5 I think there are some missing ceil operators
* There are some typos throughout the paper

\paragraph*{Ethics}
3. No ethic issues

\section*{Overall Assessment}
Thanks for the submission. While both reviewers like the motivation and the proposed solution, they are also concerned that the contribution is not clear at the current stage, and whether the solution is practical in real-world settings. The authors are encouraged to address the comments in the next iteration of the paper.

% \end{document}
